FAMuS: Frames Across Multiple Sources

Understanding event descriptions is a central aspect of language processing, but current approaches focus overwhelmingly on single sentences or documents. Aggregating information about an event \emph{across documents} can offer a much richer understanding. To this end, we present FAMuS, a new corpus of Wikipedia passages that \emph{report} on some event, paired with underlying, genre-diverse (non-Wikipedia) \emph{source} articles for the same event. Events and (cross-sentence) arguments in both report and source are annotated against FrameNet, providing broad coverage of different event types. We present results on two key event understanding tasks enabled by FAMuS: \emph{source validation} -- determining whether a document is a valid source for a target report event -- and \emph{cross-document argument extraction} -- full-document argument extraction for a target event from both its report and the correct source article. We release both FAMuS and our models to support further research.

==> sections/analysis.tex <==
\paragraph{Source Validation}
\begin{figure}[t]
    \centering
    \tiny
    \includegraphics[width=\columnwidth, scale=1]{figures/source_val_performance_by_source_length.png}
    \caption{Analysis of F1 Score Variations Across Different Bins of Source Lengths in the Source Validation Task.}
    \vspace{-3em}
    \label{fig:source_val_by_source_length}
\end{figure}
Table \ref{tab:source_val_results} provides a comparison of how different models prioritize precision versus recall during the source validation task. To enhance our understanding of these distinctions, we evaluated the F1 scores of the various models using the development set, further dissecting their performances across different source length bins. The organization of these bins is by their respective percentiles: the 10th, 25th, 50th, 75th, and beyond the 90th percentile.

As illustrated in Figure \ref{fig:source_val_by_source_length}, ChatGPT performs exceptionally well in the shortest source length bin, achieving an F1 score of 84. However, as the source length extends, the performance of ChatGPT diminishes noticeably, indicating a potential limitation in handling longer text inputs. Contrastingly, the Longformer model exhibits remarkable consistency across all source length bins. Except for the smallest bin, it sustains an F1 score above 75, irrespective of the increase in source length. This emphasizes the proficiency of the Longformer model in dealing with tasks involving a wide range of source lengths.

\begin{figure}[t]
    \centering
    \tiny
    \includegraphics[width=\columnwidth, scale=1]{figures/cdae_performance_by_source_length.png}
    \caption{Analysis of $\text{CEAF-RME}_a$ F1 Score across different Bins of Source Lengths in the CDAE Task (Source). The Iter-X model used here is IterX\textsubscript{pred} which does not have access to gold spans.}
    \vspace{-3em}
    \label{fig:cdae_by_source_length}
\end{figure}
\paragraph{Cross Document Argument Extraction}
Similar to the Source Validation analysis, we also analyze the model performance on Source Data based on the source length bins. Across all models, it is seen that the performance degrades as the source length increases (Figure \ref{fig:cdae_by_source_length}).
